The impact when neural min-sum variant meets ordered statistics decoding of LDPC codes

This paper introduces three key initiatives in the pursuit of a hybrid decoding framework characterized by superior decoding performance, high throughput, low complexity, and independence from channel noise variance. Firstly, adopting a graphical neural network perspective, we propose a design methodology for a family of neural min-sum variants. Our exploration delves into the frame error rates associated with different decoding variants and the consequential impact of decoding failures on subsequent ordered statistics decoding. Notably, these neural min-sum variants exhibit generally indistinguishable performance, hence the simplest member is chosen as the constituent of the hybrid decoding. Secondly, to address computational complexities arising from exhaustive searches for authentic error patterns in cases of decoding failure, two alternatives for ordered statistics decoding implementation are proposed. The first approach involves uniformly grouping test error patterns, while the second scheme dynamically generates qualified searching test error patterns with varied sizes for each group. In both methods, group priorities are determined empirically. Thirdly, iteration diversity is highlighted in the case of LDPC codes requiring high maximum iterations of decoding. This is achieved by segmenting the long iterative decoding trajectory of a decoding failure into shorter segments, which are then independently fed to small models to enhance the chances of acquiring the authentic error pattern. These ideas are substantiated through extensive simulation results covering the codes with block lengths ranging from one hundred to several hundreds.

==> plots/fer_code.tex <==
# -*- coding: utf-8 -*-
"""
Created on Tue Sep 26 22:34:17 2023

@author: Administrator
"""
# -*- coding: utf-8 -*-
"""
Created on Wed Sep 13 07:39:41 2023

@author: lgw
"""
#wimax(1056,880)  3.0-3.8-0.1dB, NMS-2(16)
ldpc_testing_fer = [(3.0,0.5149),(3.1,0.3927),(3.2,0.2836),(3.3,0.1948),(3.4,0.1263),(3.5,0.0772),(3.6,0.0424),(3.7,0.0232),(3.8,0.0116)]
#wimax(1056,880)  3.0-3.8-0.1dB, NMS-2(16) non-DIA,order-3,dynamic
osd_fer1 = [(3.0,0.3413),(3.1,0.2481),(3.2,0.2137),(3.3,0.1527),(3.4,0.1224),(3.5,0.1105)]
#wimax(1056,880)  3.0-3.8-0.1dB, NMS-2(16) DIA order-3,dynamic
osd_fer2 = [(3.0,0.2309),(3.1,0.2),(3.2,0.1393),(3.3,0.0986),(3.4,0.083),(3.5,0.0557)]

osd_fer_order_list = [osd_fer1,osd_fer2]
order_fer_list = []
for k in range(2):
    order_fer = [round(ldpc_testing_fer[i][1]*osd_fer_order_list[k][i][1],4) for i in range(len(ldpc_testing_fer[:6]))]
    order_fer_list.append(order_fer)
    print(order_fer)
print('gameover')
###########################order-3##########################################
#wimax(1056,880)  3.0-3.8-0.1dB, NMS-2(16) DIA order-3,dynamic
# For 3.0dB (order_sum:3) summary:
# ----> S:333 F:100
# FER:0.2309 Average candidate size:227565.649
# For 3.1dB (order_sum:3) summary:
# ----> S:400 F:100
# FER:0.2 Average candidate size:229475.064
# For 3.2dB (order_sum:3) model_cnn-dynamic:
# ----> S:618 F:100
# FER:0.1393 Average candidate size: 223529.8064 
# For 3.3dB (order_sum:3) model_cnn-dynamic:
# ----> S:914 F:100
# FER:0.0986 Average candidate size: 223644.9024 
# For 3.4dB (order_sum:3) summary:
# --> S/F: 1018 / 92 
# FER: 0.083 Average size: 221622.1306
# For 3.5dB (order_sum:3) summary:
# ----> S:1442 F:85
# FER:0.0557 Average candidate size:218008.4905

#wimax(1056,880)  3.0-3.8-0.1dB, NMS-2(16) non-DIA,order-3,dynamic
# For 3.0dB (order_sum:3) benchmark-dynamic:
# ----> S:193 F:100
# FER:0.3413 Average candidate size: 223720.6075 
# For 3.1dB (order_sum:3) benchmark-dynamic:
# ----> S:303 F:100
# FER:0.2481 Average candidate size: 224253.3821 
# For 3.2dB (order_sum:3) benchmark-dynamic:
# ----> S:368 F:100
# FER:0.2137 Average candidate size: 222701.3462 
# For 3.3dB (order_sum:3) benchmark-dynamic:
# ----> S:555 F:100
# FER:0.1527 Average candidate size: 217946.9588 
# For 3.4dB (order_sum:3) summary:
# --> S/F: 667 / 93  
# FER: 0.1224 Average size: 217923.0092
# For 3.5dB (order_sum:3) summary:
# ----> S:805 F:100
# FER:0.1105 Average candidate size:212342.8265


#CCSDS(128,64) 2.0-3.0-0.2dB, non-DIA,order-3,fixed
# For 2.0dB (order_sum:3) summary:
# ----> S:4899 F:201
# FER:0.0394 Average candidate size:43745.0
# For 2.2dB (order_sum:3) summary:
# ----> S:7700 F:200
# FER:0.0253 Average candidate size:43745.0
# For 2.4dB (order_sum:3) summary:
# --> S/F: 7860 / 140 Average size: 43745.0
# For 2.6dB (order_sum:3) summary:
# --> S/F: 11821 / 179 Average size: 43745.0
# For 2.8dB (order_sum:3) summary:
# --> S/F: 8905 / 95 Average size: 43745.0
# For 3.0dB (order_sum:3) summary:
# --> S/F: 7954 / 46  Average size: 43745.0

# #CCSDS(128,64) 2.0-3.0-0.2dB, DIA,order-3,fixed
# For 2.0dB (order_sum:3) summary:
# ----> S:8400 F:200
# FER:0.0233 Average candidate size:43745.0
# For 2.2dB (order_sum:3) summary:
# --> S/F: 7873 / 127  Average size: 43745.0
# For 2.4dB (order_sum:3) summary:
# --> S/F: 16846 / 154  Average size: 43745.0
# For 2.6dB (order_sum:3) summary:
# --> S/F: 8938 / 62 Average size: 43745.0
# For 2.8dB (order_sum:3) summary:
# --> S/F: 9967 / 33  Average size: 43745.0
# For 3.0dB (order_sum:3) summary:
# --> S/F: 11974 / 26  Average size: 43745.0

# #CCSDS(128,64) 2.6-3.2-0.2dB, non-DIA,order-3,dynamic
# For 2.0dB (order_sum:3) benchmark-dynamic:
# ----> S:4299 F:201
# FER:0.0447 Average candidate size: 24263.9527
# For 2.2dB (order_sum:3) summary:
# ----> S:5698 F:202
# FER:0.0342 Average candidate size:24144.0536
# For 2.4dB (order_sum:3) summary:
# ----> S:8199 F:201
# FER:0.0239 Average candidate size:23977.3589
# For 2.6dB (order_sum:3) summary:
# ----> S:25567 F:447
# FER:0.0172 Average candidate size:23708.6651
# For 2.8dB (order_sum:3) summary:
# ----> S:22525 F:281
# FER:0.0123 Average candidate size:23491.5317
# For 3.0dB (order_sum:3) summary:
# ----> S:15916 F:154
# FER:0.0096 Average candidate size:23277.1724
# For 3.2dB (order_sum:3) summary:
# ----> S:13438 F:120
# FER:0.0089 Average candidate size:23041.983
# For 3.4dB (order_sum:3) summary:
# ----> S:8526 F:50
# FER:0.0058 Average candidate size:22721.7825
# For 3.6dB (order_sum:3) summary:
# ----> S:6846 F:35
# FER:0.0051 Average candidate size:22439.3058

# #CCSDS(128,64) 2.6-3.2-0.2dB, DIA,order-3,dynamic
# For 2.0dB (order_sum:3) model_cnn-dynamic:
# ----> S:5999 F:201
# FER:0.0324 Average candidate size: 13290.3511 
# For 2.2dB (order_sum:3) summary:
# --> S/F: 8820 / 180  Average size: 13365.1762
# For 2.4dB (order_sum:3) model_cnn-dynamic:
# ----> S:16299 F:201
# FER:0.0122 Average candidate size: 13443.4167 
# For 2.6dB (order_sum:3) summary:
# ----> S:25796 F:218
# FER:0.0084 Average candidate size:13442.3844
# For 2.8dB (order_sum:3) dynamicmodel_cnn:
# ----> S:22678 F:128
# FER:0.0056 Average candidate size: 13376.605 
# For 3.0dB (order_sum:3) summary:
# ----> S:16024 F:46
# FER:0.0029 Average candidate size:13455.4973

# ###########################order-2##########################################
# #CCSDS(128,64) 2.6-3.6-0.2dB non-DIA,order-2,fixed
# For 2.6dB (order_sum:2) summary:
# ----> S:4600 F:200
# FER:0.0417 Average candidate size:2081.0
# For 2.8dB (order_sum:2) summary:
# ----> S:6899 F:201
# FER:0.0283 Average candidate size:2081.0
# For 3.0dB (order_sum:2) summary:
# ----> S:8999 F:201
# FER:0.0218 Average candidate size:2081.0
# For 3.2dB (order_sum:2) summary:
# ----> S:8900 F:200
# FER:0.022 Average candidate size:2081.0
# For 3.4dB (order_sum:2) summary:
# ----> S:8436 F:140
# FER:0.0163 Average candidate size:2081.0
# For 3.6dB (order_sum:2) summary:
# ----> S:6798 F:83
# FER:0.0121 Average candidate size:2081.0

# #CCSDS(128,64) 2.6-3.6-0.2dB DIA,order-2,fixed
# For 2.6dB (order_sum:2) summary:
# ----> S:8899 F:201
# FER:0.0221 Average candidate size:2081.0
# For 2.8dB (order_sum:2) summary:
# ----> S:14600 F:200
# FER:0.0135 Average candidate size:2081.0
# For 3.0dB (order_sum:2) summary:
# ----> S:15936 F:134
# FER:0.0083 Average candidate size:2081.0
# For 3.2dB (order_sum:2) summary:
# ----> S:13484 F:74
# FER:0.0055 Average candidate size:2081.0
# For 3.4dB (order_sum:2) summary:
# ----> S:8534 F:42
# FER:0.0049 Average candidate size:2081.0
# For 3.6dB (order_sum:2) summary:
# ----> S:6861 F:20
# FER:0.0029 Average candidate size:2081.0

# #CCSDS(128,64) 2.6-3.6-0.2dB non-DIA,order-2,dynamic
# osd_fer3 = [0.0385,0.0263,0.0224,0.0227,0.0168,0.0121]

# For 2.6dB (order_sum:2) summary:
# ----> S:4597 F:203
# FER:0.0423 Average candidate size:1910.1402
# For 2.8dB (order_sum:2) summary:
# ----> S:6798 F:202
# FER:0.0289 Average candidate size:1896.1763
# For 3.0dB (order_sum:2) summary:
# ----> S:8998 F:202
# FER:0.022 Average candidate size:1883.9201
# For 3.2dB (order_sum:2) summary:
# ----> S:8499 F:201
# FER:0.0231 Average candidate size:1879.3506
# For 3.4dB (order_sum:2) summary:
# ----> S:8431 F:145
# FER:0.0169 Average candidate size:1854.3572
# For 3.6dB (order_sum:2) summary:
# ----> S:6792 F:89
# FER:0.0129 Average candidate size:1843.9965

# #CCSDS(128,64) 2.6-3.6-0.2dB DIA,order-2,dynamic
# For 2.6dB (order_sum:2) summary:
# ----> S:8700 F:200
# FER:0.0225 Average candidate size:1822.9436
# For 2.8dB (order_sum:2) summary:
# ----> S:14500 F:200
# FER:0.0136 Average candidate size:1813.4623
# For 3.0dB (order_sum:2) summary:
# ----> S:15932 F:138
# FER:0.0086 Average candidate size:1813.0834
# For 3.2dB (order_sum:2) summary:
# ----> S:13483 F:75
# FER:0.0055 Average candidate size:1804.9164
# For 3.4dB (order_sum:2) summary:
# ----> S:8534 F:42
# FER:0.0049 Average candidate size:1786.0169
# For 3.6dB (order_sum:2) summary:
# ----> S:6861 F:20
# FER:0.0029 Average candidate size:1783.8872

[0.1757, 0.0974, 0.0606, 0.0297, 0.0155, 0.0085]
[0.1189, 0.0785, 0.0395, 0.0192, 0.0105, 0.0043]





==> sections/ackowledgment.tex <==
\section*{Acknowledgment}
%\section{Acknowledgment}
The authors would like to thank Alphabet Inc. for providing the excellent computing platforms of Colab and Kaggle online, which make it possible to debug, train and test our models freely. Thanks are also given to the anonymous reviewers for providing their valuable feedback in improving the quality of this paper.

==> sections/cover_letter.tex <==
Dear [Editor's Name],

I hope this letter finds you well. We are submitting our manuscript titled "A Hybrid Framework of Neural Min-Sum Variant and Ordered Statistical Decoding for LDPC Codes" for your consideration.

In this paper, we present a hybrid framework that combines a neural min-sum (NMS) variant with ordered statistical decoding (OSD) for the efficient decoding of LDPC codes. Our proposed framework offers superior decoding performance, low complexity, and channel invariance. A key highlight is its remarkable data throughput. The NMS variant efficiently handles the majority of the decoding load in parallel, while the OSD component is dedicated to processing the few NMS decoding failures. Despite the inherently serial nature of OSD, our framework adeptly mitigates bottlenecks that typically arise from the mismatch between parallel and serial processing speeds.

In terms of implementation details, we provide an intuitive interpretation of the NMS variants within the context of graphical neural networks. We empirically conclude that the simplest NMS variant proves to be the most effective. We also introduce two alternatives for generating searching test error patterns for the OSD component, which significantly influences its complexity. Furthermore, we propose iteration diversity as a means to enhance decoding performance and reduce model complexity by segmenting the long iteration trajectory of decoding failures.

Our empirical simulations, conducted on three LDPC codes with short to moderate block lengths, validate the effectiveness of our proposed designs. In conclusion, this paper offers promising insights into achieving near maximum likelihood decoding at a feasible complexity for LDPC codes.

We believe our work aligns with the scope and interests of [Journal Name], and we hope you find it suitable for publication. We appreciate your time and consideration.

Thank you for your attention, and we look forward to your favorable response.

Sincerely,

[Your Full Name]
[Your Affiliation]
[Your Contact Information]
